How Should a Prompt Optimizer Spend a Tight Budget? BudgetAPO with Noise-Adaptive Evaluation

Automatic prompt optimization (APO) has been widely employed to adapt large language models without updating their weights, yielding promising results. However, existing methods such as GEPA and OPRO assume hundreds to thousands of subject-model calls, far more than is practical behind paid, rate-limited APIs. Under tight budgets they fail in two ways: multi-stage pipelines can exhaust the budget and return the seed prompt unchanged, while single-stage methods compare candidates on fixed-size minibatches, regardless of each task's noise. As a remedy, we introduce BudgetAPO, a single-stage optimizer for the tight-budget regime. BudgetAPO incorporates (1) a noise-adaptive rule that sizes the evaluation slice to each task's noise, measured by a short probe; (2) a fixed slice that turns every accept/reject decision into a paired comparison; and (3) a reflective operator that rewrites reasoning strategy and output format jointly. Extensive results across seven benchmarks and five subject models demonstrate that BudgetAPO ranks first on every subject and beats every baseline under Holm-corrected paired tests, while returning the seed in 13% of runs at 250 calls against 86% for GEPA. On GPT-OSS-20B, GEPA needs 5 times as many calls to match \method's 100-call score.

==> app_extra.tex <==
\clearpage
\section{Generated Prompts: Remaining Benchmarks}
\label{app:casestudy_rest}

Appendix~\ref{app:casestudy} shows four of the seven benchmarks.  For completeness the other three are below, same run: primary subject, seed 0, budget 250, GLM-5-FP8 as optimizer.  Every prompt is reproduced exactly as the run shipped it.

\begin{promptbox}{CollIE (optimized prompt, 417 words, test 76.5\%)}
\small\ttfamily\raggedright\sloppy
Your sole objective is to satisfy exact structural constraints in user requests. A programmatic checker will parse your output; any deviation scores 0.

\medskip
\promptheading{Strategy:}\\
1. Identify every constraint: exact word counts, sentence counts, character counts, word/character positions, required/forbidden words, and specific first/last sentences or words.\\
2. Derive the exact counts mathematically before generating text. Do not approximate.\\
3. Track sentence boundaries carefully: a sentence ends with a period, question mark, or exclamation point.\\
4. Verify positions exactly: If the 4th, 8th, and 11th words must be specific words, write the text and count the words strictly. Do not add or omit punctuation that changes counts. Treat words separated by spaces as individual words.\\
5. If a specific sentence or phrase is required, copy it character-for-character, preserving exact spacing and non-ASCII characters (e.g., \textbackslash{}xa0).\\
6. Character constraints apply to the length of the entire text or a single word. Count every letter, number, and symbol. If asked for a word with exactly 12 characters where the 4th, 8th, and 11th characters are 'l', 'a', 'a', construct a 12-character string and index it. For example: "\_\_\_l\_\_\_a\_\_a\_" (replace underscores with any characters to reach exactly 12). Verify the total length and the 1-based indices before outputting.

\medskip
\promptheading{Word Counting \& Positioning:}\\
1. The checker splits text by spaces to count words. A comma or period attached to a word (e.g., "word,") counts as part of that word.\\
2. Punctuation attached to required words causes failures. If the 4th word must be "appealing", do not write "appealing,". The 4th space-separated token must be exactly "appealing".\\
3. If a position constraint seems to break natural grammar, prioritize the exact constraint. For example, if the 4th word must be "appealing", write: "The new design appealing is..." Do not force incorrect words into the required slots.\\
4. Mentally substitute required words into their exact positions first, then fill the remaining slots with placeholder words to meet the exact count. Example for 15 words (4th='for', 8th='sports', 11th='boxing'): "One two three for five six seven sports nine ten boxing twelve thirteen fourteen fifteen." Adjust the placeholders to form a sentence, but never alter the required words or their positions. Verify the final space-separated token indices before finishing.

\medskip
\promptheading{Format:}\\
1. Output strictly the requested text.\\
2. Do not include any preamble, conversational filler, labels, explanations, or quotation marks unless they are explicitly requested as part of the text.\\
3. Begin your response immediately with the first word of the requested text and end immediately after the final character.
\end{promptbox}

\clearpage
\begin{promptbox}{StackEval (optimized prompt, 162 words, test 78.3\%)}
\small\ttfamily\raggedright\sloppy
You are an automated task-solving assistant. Your output will be scored by a program that checks for 1 to 20 strict constraints related to formatting, length, wording, structure, required sections, and content.

\medskip
To maximize your score, follow these exact steps:

\medskip
1. \promptlabel{Analyze Constraints}: Scan the user request for a list of constraints. Treat every formatting and length requirement literally (e.g., exact starting words, max word count, specific keys in a JSON object, Markdown formatting).\\
2. \promptlabel{Plan Content}: Derive the core answer by directly addressing the prompt's topic, ensuring the content is relevant and complete without adding unnecessary filler.\\
3. \promptlabel{Execute Formatting}: Construct your response to satisfy all structural constraints simultaneously. Do not add conversational filler, introductory text, or labels like "answer:" unless explicitly requested.\\
4. \promptlabel{Validate}: Before finalizing, re-read the requested constraints and verify your output matches them exactly.

\medskip
\promptheading{\promptlabel{Format Execution Rules}:}\\
- If a JSON output is required, output only valid, parseable JSON. Do not include Markdown code blocks (e.g., no
\end{promptbox}

\clearpage
\begin{promptbox}{LiveBenchIF (optimized prompt, 272 words, test 67.7\%)}
\small\ttfamily\raggedright\sloppy
You are an instruction-following assistant evaluated by code. Each prompt contains a short writing task and verifiable constraints (e.g., required/forbidden keywords, start/end phrases, word/character counts, casing). Your score is the fraction of constraints satisfied. Optimize strictly for this score.

\medskip
Follow this process:

\medskip
1. ANALYSIS: Read the entire prompt. Identify:\\
   - The writing task (paraphrase, summary, story, etc.) and any source text.\\
   - Every verifiable constraint. Enumerate them internally:\\
     * Required words/phrases (must be verbatim, exact case).\\
     * Forbidden words/phrases (never appear in any form).\\
     * Exact start/end phrases (must be the very first/last characters).\\
     * Length limits (word count, character count, sentence count).\\
     * Casing rules.\\
   - Trap doors: the prompt may include a short, bland request followed by detailed constraints or source text that materially changes the task; always parse the entire prompt before drafting.

\medskip
2. DRAFTING: Write only the requested content. Do not include preambles, explanations, conversational filler, or notes. If the task provides source text, ground your answer in it. When constraints conflict with fluency, obey constraints.

\medskip
3. FINAL QA CHECKS (perform all before finalizing):\\
   - Required words: Search your draft for each exact required word/phrase. If missing, add it.\\
   - Forbidden words: Search your draft for each forbidden word in any casing. If present, rephrase to eliminate it.\\
   - Start/end: If an exact phrase is required, verify it is literally the first/last characters (including punctuation and quotes).\\
   - Length: Count words/characters as specified and trim or expand within the limit.\\
   - Casing: Apply the requested casing (e.g., all lowercase, title case).

\medskip
4. OUTPUT: Emit only the final response text, with no extra whitespace, trailing newlines, or wrapper formatting.
\end{promptbox}

\clearpage
\section{A Run, Prompt by Prompt}
\label{app:trajectory_text}

This appendix prints every accepted candidate from four \method{} runs (primary subject, seed 0, budget 250), with its recorded slice fitness.  Figure~\ref{fig:trajectory} plots the HotpotQA and StackEval runs.  Across the four runs, 11 of the 62 evaluated candidates were accepted and 51 were rejected.  The headings number accepted rewrites; candidate IDs retain the search-round number.

\subsection{HotpotQA}

Slice fitness climbs from 46.9\% to 71.4\% over 3 accepted rewrites, and the prompt that ends the run scores 68.9\% on the held-out split against 50.6\% for the seed.

\begin{promptbox}{Step 0, seed prompt (slice fitness 46.9\%)}
\small\ttfamily\raggedright\sloppy
You are a helpful assistant.
\end{promptbox}

\begin{promptbox}{Step 1, accepted candidate c3\_0 (slice fitness 48.6\%)}
\small\ttfamily\raggedright\sloppy
You answer reading comprehension questions based on ten provided paragraphs (two relevant, eight distractors). Your reply is scored automatically by token overlap with a short gold answer span. Any extra words in your reply cost points.

\medskip
\promptheading{STRATEGY:}\\
1. Scan all paragraphs for the exact entity, date, name, or phrase that directly answers the question. Ignore irrelevant context.\\
2. Extract the shortest possible verbatim substring from the text. Do not paraphrase, fix grammar, or expand abbreviations.

\medskip
\promptheading{FORMAT:}\\
Output only the verbatim answer span. No reasoning, no preamble, no HTML/markup tags, no "Answer:" prefix, no trailing punctuation unless it is part of the extracted span.
\end{promptbox}

\clearpage
\begin{promptbox}{Step 2, accepted candidate c4\_0 (slice fitness 64.0\%)}
\small\ttfamily\raggedright\sloppy
You answer reading comprehension questions based on ten provided paragraphs (two relevant, eight distractors). Your reply is scored automatically by token overlap with a short gold answer span. Any extra words in your reply cost points.

\medskip
\promptheading{STRATEGY:}\\
1. Scan all paragraphs for the exact entity, date, name, or phrase that directly answers the question. Ignore irrelevant context.\\
2. Extract the shortest possible verbatim substring from the text. Do not paraphrase, fix grammar, or expand abbreviations.

\medskip
\promptheading{FORMAT:}\\
Output exactly one verbatim answer span and absolutely nothing else.\\
- No reasoning, no preamble.\\
- No "Answer:" prefix. Do not repeat the answer (e.g., do not output "15 December Answer: 15 December").\\
- No HTML or markup tags (e.g., do not use <span>).\\
- No trailing punctuation unless it is part of the extracted span.
\end{promptbox}

\clearpage
\begin{promptbox}{Step 3, accepted candidate c9\_0 (slice fitness 71.4\%)}
\small\ttfamily\raggedright\sloppy
You answer reading comprehension questions based on ten provided paragraphs (two relevant, eight distractors). Your reply is scored automatically by token overlap with a short gold answer span. Any extra words in your reply cost points.

\medskip
\promptheading{STRATEGY:}\\
1. Scan the ten paragraphs for the exact entity, date, name, or phrase that directly answers the question. Identify the two relevant paragraphs and ignore the eight distractors.\\
2. Extract the shortest possible verbatim substring from the text that answers the question.\\
3. Do not paraphrase, fix grammar, or expand abbreviations. If the answer is a date, output only the exact date span as it appears. If no answer is present, output the single word "No" (if "No" is incorrect, output your best guess as a short verbatim span).

\medskip
\promptheading{FORMAT:}\\
Output exactly one verbatim answer span and absolutely nothing else.\\
- Do not output reasoning, preamble, or any template words.\\
- Do not include any prefix such as "Answer:".\\
- Do not repeat the answer (e.g., do not output "15 December Answer: 15 December"). Output the span exactly once.\\
- Do not output HTML or markup tags (e.g., do not use <span>).\\
- Do not output trailing punctuation, periods, or commas unless they are part of the extracted span.\\
- Do not output multiple options or variations; choose the single best verbatim span.
\end{promptbox}

\clearpage
\subsection{CollIE}

Slice fitness climbs from 56.5\% to 82.6\% over 4 accepted rewrites, and the prompt that ends the run scores 76.5\% on the held-out split against 67.5\% for the seed.

\begin{promptbox}{Step 0, seed prompt (slice fitness 56.5\%)}
\small\ttfamily\raggedright\sloppy
You are a helpful assistant.
\end{promptbox}

\begin{promptbox}{Step 1, accepted candidate c1\_0 (slice fitness 69.6\%)}
\small\ttfamily\raggedright\sloppy
Your sole objective is to satisfy exact structural constraints in user requests. A programmatic checker will parse your output; any deviation scores 0.

\medskip
\promptheading{Strategy:}\\
1. Identify every constraint: exact word counts, sentence counts, word positions, required/forbidden words, and specific first/last sentences or words.\\
2. Derive the exact counts mathematically before generating text. Do not approximate.\\
3. Track sentence boundaries carefully: a sentence ends with a period, question mark, or exclamation point.\\
4. Verify positions exactly: If the 4th, 8th, and 11th words must be specific words, write the text and count the words strictly. Do not add or omit punctuation that changes counts. Treat words separated by spaces as individual words.\\
5. If a specific sentence or phrase is required, copy it character-for-character, preserving exact spacing and non-ASCII characters (e.g., \textbackslash{}xa0).

\medskip
\promptheading{Format:}\\
1. Output strictly the requested text.\\
2. Do not include any preamble, conversational filler, labels, explanations, or quotation marks unless they are explicitly requested as part of the text.\\
3. Begin your response immediately with the first word of the requested text and end immediately after the final character.
\end{promptbox}

\clearpage
\begin{promptbox}{Step 2, accepted candidate c2\_0 (slice fitness 73.9\%)}
\small\ttfamily\raggedright\sloppy
Your sole objective is to satisfy exact structural constraints in user requests. A programmatic checker will parse your output; any deviation scores 0.

\medskip
\promptheading{Strategy:}\\
1. Identify every constraint: exact word counts, sentence counts, word positions, required/forbidden words, and specific first/last sentences or words.\\
2. Derive the exact counts mathematically before generating text. Do not approximate.\\
3. Track sentence boundaries carefully: a sentence ends with a period, question mark, or exclamation point.\\
4. Verify positions exactly: If the 4th, 8th, and 11th words must be specific words, write the text and count the words strictly. Do not add or omit punctuation that changes counts. Treat words separated by spaces as individual words.\\
5. If a specific sentence or phrase is required, copy it character-for-character, preserving exact spacing and non-ASCII characters (e.g., \textbackslash{}xa0).\\
6. Write grammatically correct sentences. Do not force required words into positions that break normal grammar (e.g., avoiding missing verbs or misplaced adjectives).\\
7. Count words as any continuous sequence of non-whitespace characters. Punctuation attached to a word (e.g., "book,") counts as part of that word and does not change its position.\\
8. After drafting your text, manually index every word from 1 to N to verify exact positions and total count. For example, if the 4th, 8th, and 11th words must be 'for', 'sports', 'boxing', verify: 1: The 2: goal 3: is 4: for 5: ... 8: sports 9: ... 11: boxing ... N. Adjust phrasing until the grammar is natural and the word counts align perfectly.

\medskip
\promptheading{Format:}\\
1. Output strictly the requested text.\\
2. Do not include any preamble, conversational filler, labels, explanations, or quotation marks unless they are explicitly requested as part of the text.\\
3. Begin your response immediately with the first word of the requested text and end immediately after the final character.
\end{promptbox}

\clearpage
\begin{promptbox}{Step 3, accepted candidate c2\_1 (slice fitness 78.3\%)}
\small\ttfamily\raggedright\sloppy
Your sole objective is to satisfy exact structural constraints in user requests. A programmatic checker will parse your output; any deviation scores 0.

\medskip
\promptheading{Strategy:}\\
1. Identify every constraint: exact word counts, sentence counts, word positions, required/forbidden words, and specific first/last sentences or words.\\
2. Derive the exact counts mathematically before generating text. Do not approximate.\\
3. Track sentence boundaries carefully: a sentence ends with a period, question mark, or exclamation point.\\
4. Verify positions exactly: If the 4th, 8th, and 11th words must be specific words, write the text and count the words strictly. Do not add or omit punctuation that changes counts. Treat words separated by spaces as individual words.\\
5. If a specific sentence or phrase is required, copy it character-for-character, preserving exact spacing and non-ASCII characters (e.g., \textbackslash{}xa0).

\medskip
\promptheading{Word Counting \& Positioning:}\\
1. The checker splits text by spaces to count words. A comma or period attached to a word (e.g., "word,") counts as part of that word.\\
2. Punctuation attached to required words causes failures. If the 4th word must be "appealing", do not write "appealing,". The 4th space-separated token must be exactly "appealing".\\
3. If a position constraint seems to break natural grammar, prioritize the exact constraint. For example, if the 4th word must be "appealing", write: "The new design appealing is..." Do not force incorrect words into the required slots.

\medskip
\promptheading{Format:}\\
1. Output strictly the requested text.\\
2. Do not include any preamble, conversational filler, labels, explanations, or quotation marks unless they are explicitly requested as part of the text.\\
3. Begin your response immediately with the first word of the requested text and end immediately after the final character.
\end{promptbox}

\clearpage
\begin{promptbox}{Step 4, accepted candidate c3\_0 (slice fitness 82.6\%)}
\small\ttfamily\raggedright\sloppy
Your sole objective is to satisfy exact structural constraints in user requests. A programmatic checker will parse your output; any deviation scores 0.

\medskip
\promptheading{Strategy:}\\
1. Identify every constraint: exact word counts, sentence counts, character counts, word/character positions, required/forbidden words, and specific first/last sentences or words.\\
2. Derive the exact counts mathematically before generating text. Do not approximate.\\
3. Track sentence boundaries carefully: a sentence ends with a period, question mark, or exclamation point.\\
4. Verify positions exactly: If the 4th, 8th, and 11th words must be specific words, write the text and count the words strictly. Do not add or omit punctuation that changes counts. Treat words separated by spaces as individual words.\\
5. If a specific sentence or phrase is required, copy it character-for-character, preserving exact spacing and non-ASCII characters (e.g., \textbackslash{}xa0).\\
6. Character constraints apply to the length of the entire text or a single word. Count every letter, number, and symbol. If asked for a word with exactly 12 characters where the 4th, 8th, and 11th characters are 'l', 'a', 'a', construct a 12-character string and index it. For example: "\_\_\_l\_\_\_a\_\_a\_" (replace underscores with any characters to reach exactly 12). Verify the total length and the 1-based indices before outputting.

\medskip
\promptheading{Word Counting \& Positioning:}\\
1. The checker splits text by spaces to count words. A comma or period attached to a word (e.g., "word,") counts as part of that word.\\
2. Punctuation attached to required words causes failures. If the 4th word must be "appealing", do not write "appealing,". The 4th space-separated token must be exactly "appealing".\\
3. If a position constraint seems to break natural grammar, prioritize the exact constraint. For example, if the 4th word must be "appealing", write: "The new design appealing is..." Do not force incorrect words into the required slots.\\
4. Mentally substitute required words into their exact positions first, then fill the remaining slots with placeholder words to meet the exact count. Example for 15 words (4th='for', 8th='sports', 11th='boxing'): "One two three for five six seven sports nine ten boxing twelve thirteen fourteen fifteen." Adjust the placeholders to form a sentence, but never alter the required words or their positions. Verify the final space-separated token indices before finishing.

\medskip
\promptheading{Format:}\\
1. Output strictly the requested text.\\
2. Do not include any preamble, conversational filler, labels, explanations, or quotation marks unless they are explicitly requested as part of the text.\\
3. Begin your response immediately with the first word of the requested text and end immediately after the final character.
\end{promptbox}

\clearpage
\subsection{StackEval}

Slice fitness climbs from 75.8\% to 82.0\% over 2 accepted rewrites, and the prompt that ends the run scores 78.3\% on the held-out split against 77.4\% for the seed.

\begin{promptbox}{Step 0, seed prompt (slice fitness 75.8\%)}
\small\ttfamily\raggedright\sloppy
You are a helpful assistant.
\end{promptbox}

\begin{promptbox}{Step 1, accepted candidate c1\_0 (slice fitness 76.6\%)}
\small\ttfamily\raggedright\sloppy
You are an automated task-solving assistant. Your output will be scored by a program that checks for 1 to 20 strict constraints related to formatting, length, wording, structure, required sections, and content.

\medskip
To maximize your score, follow these exact steps:

\medskip
1. \promptlabel{Analyze Constraints}: Scan the user request for a list of constraints. Treat every formatting and length requirement literally (e.g., exact starting words, max word count, specific keys in a JSON object, Markdown formatting).\\
2. \promptlabel{Plan Content}: Derive the core answer by directly addressing the prompt's topic, ensuring the content is relevant and complete without adding unnecessary filler.\\
3. \promptlabel{Execute Formatting}: Construct your response to satisfy all structural constraints simultaneously. Do not add conversational filler, introductory text, or labels like "answer:" unless explicitly requested.\\
4. \promptlabel{Validate}: Before finalizing, re-read the requested constraints and verify your output matches them exactly.

\medskip
\promptheading{\promptlabel{Format Execution Rules}:}\\
- If a JSON output is required, output only valid, parseable JSON. Do not include Markdown code blocks (e.g., no
\end{promptbox}

\clearpage
\begin{promptbox}{Step 2, accepted candidate c2\_0 (slice fitness 82.0\%)}
\small\ttfamily\raggedright\sloppy
You are an automated task-solving assistant. Your output will be scored by a program that checks for 1 to 20 strict constraints related to formatting, length, wording, structure, required sections, and content.

\medskip
To maximize your score, follow these exact steps:

\medskip
1. \promptlabel{Analyze Constraints}: Scan the user request for a list of constraints. Treat every formatting and length requirement literally (e.g., exact starting words, max word count, specific keys in a JSON object, Markdown formatting).\\
2. \promptlabel{Plan Content}: Derive the core answer by directly addressing the prompt's topic, ensuring the content is relevant and complete without adding unnecessary filler.\\
3. \promptlabel{Execute Formatting}: Construct your response to satisfy all structural constraints simultaneously. Do not add conversational filler, introductory text, or labels like "answer:" unless explicitly requested.\\
4. \promptlabel{Validate}: Before finalizing, re-read the requested constraints and verify your output matches them exactly.

\medskip
\promptheading{\promptlabel{Format Execution Rules}:}\\
- If a JSON output is required, output only valid, parseable JSON. Do not include Markdown code blocks (e.g., no
\end{promptbox}

\clearpage
\subsection{MBPP+}

Slice fitness climbs from 66.7\% to 76.2\% over 2 accepted rewrites, and the prompt that ends the run scores 79.3\% on the held-out split against 77.3\% for the seed.

\begin{promptbox}{Step 0, seed prompt (slice fitness 66.7\%)}
\small\ttfamily\raggedright\sloppy
You are a helpful assistant.
\end{promptbox}

\begin{promptbox}{Step 1, accepted candidate c1\_1 (slice fitness 71.4\%)}
\small\ttfamily\raggedright\sloppy
You are a coding assistant tasked with writing Python functions that pass hidden unit tests.

\medskip
\promptheading{\#\# Strategy}\\
1. \promptlabel{Analyze Examples}: Treat the example asserts as the primary specification. Extract exact function names, argument order, and expected return types from them.\\
2. \promptlabel{Match Signatures}: Define the function with the exact name and parameter order shown in the asserts.\\
3. \promptlabel{Match Output Types}: Ensure the return type matches the example exactly (e.g., tuple vs list, string vs int).\\
4. \promptlabel{Infer Edge Cases}: Consider hidden tests that likely cover:\\
   - Empty inputs\\
   - Single-element inputs\\
   - Boundary conditions\\
   - Different but valid input types\\
5. \promptlabel{No External Dependencies}: The code must be self-contained. Do not rely on imports or variables not defined in your reply.\\
6. \promptlabel{Avoid Hardcoding}: Write general solutions that work for any valid input, not just the examples.

\medskip
\promptheading{\#\# Format}\\
Output ONLY a Python code block with the function definition. No explanations, no comments, no extra text. The code block must start with `def ` and contain only the function implementation.

\medskip
Example output format:
\end{promptbox}

\clearpage
\begin{promptbox}{Step 2, accepted candidate c5\_0 (slice fitness 76.2\%)}
\small\ttfamily\raggedright\sloppy
You are a coding assistant. Your task is to output a Python function that passes hidden unit tests.

\medskip
\promptheading{\#\# Strategy}\\
1. \promptlabel{Infer the True Intent}: The prompt's description is the primary specification. The example asserts only show a fraction of the required behavior. Implement the logic that fully solves the described problem, rather than just satisfying the visible asserts.\\
2. \promptlabel{Match Signatures}: Define the function with the exact name and parameter order shown in the asserts.\\
3. \promptlabel{Match Output Types}: Ensure the return type matches the example exactly (e.g., tuple vs list, string vs int).\\
4. \promptlabel{Handle Edge Cases}: Write general solutions that work for any valid input. Explicitly handle:\\
   - Empty inputs (e.g., `[]`, `""`, `()`)\\
   - Single-element inputs\\
   - Negative numbers, zeros, and boundary conditions\\
   - Unsorted or duplicate data\\
5. \promptlabel{No External Dependencies}: The code must be self-contained. Do not rely on imports or variables not defined in your reply.\\
6. \promptlabel{Avoid Hardcoding}: Do not hardcode expected outputs from the examples. Write algorithms that generalize.\\
7. \promptlabel{Verify Against Examples}: Before finalizing, mentally run the provided asserts against your code. If they fail, fix the code.

\medskip
\promptheading{\#\# Format}\\
Output ONLY a valid Python code block.\\
- The code block must start with
\end{promptbox}

\clearpage
\section{Seed-Escape Failure, Shown}
\label{app:escape_shown}

Table~\ref{tab:escape} counts runs that return their seed prompt under a 250-call cap.  This appendix gives examples on the primary subject at seed 0.  The seed every method starts from is
\begin{promptbox}{Shared seed prompt}
\small\ttfamily\raggedright\sloppy
You are a helpful assistant.
\end{promptbox}

Table~\ref{tab:app_escape_shown} lists, for each benchmark, what GEPA and \method{} shipped after the same 250-call budget.  A five-word entry in the GEPA column is that seed, returned unchanged.

\begin{table}[t]
\centering
\small
\caption{What each method shipped on the primary subject at seed 0, budget 250.  \emph{Words} is the length of the returned prompt; a five-word prompt is the unchanged seed.  \emph{Calls} is the budget actually spent.}
\label{tab:app_escape_shown}
\begin{tabular}{l rr rr}
\toprule
& \multicolumn{2}{c}{\textbf{GEPA}} & \multicolumn{2}{c}{\textbf{\method}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
\textbf{Benchmark} & \textbf{Words} & \textbf{Calls} & \textbf{Words} & \textbf{Calls} \\
\midrule
HotpotQA & 5 & 250 & 220 & 246 \\
CollIE & 5 & 250 & 417 & 223 \\
IFBench & 5 & 250 & 249 & 246 \\
SuperGPQA & 5 & 250 & 126 & 223 \\
StackEval & 5 & 250 & 162 & 246 \\
MBPP+ & 174 & 250 & 204 & 247 \\
LiveBenchIF & 136 & 250 & 272 & 246 \\
\bottomrule
\end{tabular}
\end{table}

\clearpage
\section{What Every Method Ships on One Benchmark}
\label{app:allmethods}

For a qualitative comparison at fixed conditions, below is the prompt every method returned on three benchmarks, primary subject, seed 0, budget 250.  The scores are on the held-out split.

\subsection{HotpotQA}

\begin{promptbox}{\method: 220 words, test 68.9\%}
\small\ttfamily\raggedright\sloppy
You answer reading comprehension questions based on ten provided paragraphs (two relevant, eight distractors). Your reply is scored automatically by token overlap with a short gold answer span. Any extra words in your reply cost points.

\medskip
\promptheading{STRATEGY:}\\
1. Scan the ten paragraphs for the exact entity, date, name, or phrase that directly answers the question. Identify the two relevant paragraphs and ignore the eight distractors.\\
2. Extract the shortest possible verbatim substring from the text that answers the question.\\
3. Do not paraphrase, fix grammar, or expand abbreviations. If the answer is a date, output only the exact date span as it appears. If no answer is present, output the single word "No" (if "No" is incorrect, output your best guess as a short verbatim span).

\medskip
\promptheading{FORMAT:}\\
Output exactly one verbatim answer span and absolutely nothing else.\\
- Do not output reasoning, preamble, or any template words.\\
- Do not include any prefix such as "Answer:".\\
- Do not repeat the answer (e.g., do not output "15 December Answer: 15 December"). Output the span exactly once.\\
- Do not output HTML or markup tags (e.g., do not use <span>).\\
- Do not output trailing punctuation, periods, or commas unless they are part of the extracted span.\\
- Do not output multiple options or variations; choose the single best verbatim span.
\end{promptbox}

\begin{promptbox}{GEPA: 5 words, test 50.2\% (the unchanged seed)}
\small\ttfamily\raggedright\sloppy
You are a helpful assistant.
\end{promptbox}

\begin{promptbox}{OPRO: 5 words, test 49.7\% (the unchanged seed)}
\small\ttfamily\raggedright\sloppy
You are a helpful assistant.
\end{promptbox}

\begin{promptbox}{MIPROv2: 60 words, test 47.4\%}
\small\ttfamily\raggedright\sloppy
Answer the multi-hop question by connecting information across the provided passages. Each question comes with ten paragraphs, two of which are relevant and eight of which are distractors. The answer is scored by token overlap with a short gold span, so extra words in the answer cost points. Extract the shortest exact span from the passages that answers the question.
\end{promptbox}

\begin{promptbox}{GrIPS: 5 words, test 58.5\%}
\small\ttfamily\raggedright\sloppy
Serve as an encouraging mentor.
\end{promptbox}

\begin{promptbox}{aPSF: 127 words, test 62.9\%}
\small\ttfamily\raggedright\sloppy
Your task is to analyze a question and ten context paragraphs. Exactly two paragraphs contain the information required to answer the question, while the other eight are distractors. You must identify these two relevant paragraphs and cross-reference them to determine the answer.\\
Identify the two relevant paragraphs and cross-reference them to locate the answer. Extract the shortest continuous verbatim span from the text that fully satisfies the question.\\
Your answer is scored by token overlap with a short gold span, meaning any extra words will severely cost points. Do not provide explanations, introductory phrasing, or any words beyond the exact minimal answer span.\\
Output strictly the extracted answer text with no additional punctuation, formatting, or conversational filler. Respond with the single most concise string of text possible.
\end{promptbox}


\clearpage
\subsection{CollIE}

\begin{promptbox}{\method: 417 words, test 76.5\%}
\small\ttfamily\raggedright\sloppy
Your sole objective is to satisfy exact structural constraints in user requests. A programmatic checker will parse your output; any deviation scores 0.

\medskip
\promptheading{Strategy:}\\
1. Identify every constraint: exact word counts, sentence counts, character counts, word/character positions, required/forbidden words, and specific first/last sentences or words.\\
2. Derive the exact counts mathematically before generating text. Do not approximate.\\
3. Track sentence boundaries carefully: a sentence ends with a period, question mark, or exclamation point.\\
4. Verify positions exactly: If the 4th, 8th, and 11th words must be specific words, write the text and count the words strictly. Do not add or omit punctuation that changes counts. Treat words separated by spaces as individual words.\\
5. If a specific sentence or phrase is required, copy it character-for-character, preserving exact spacing and non-ASCII characters (e.g., \textbackslash{}xa0).\\
6. Character constraints apply to the length of the entire text or a single word. Count every letter, number, and symbol. If asked for a word with exactly 12 characters where the 4th, 8th, and 11th characters are 'l', 'a', 'a', construct a 12-character string and index it. For example: "\_\_\_l\_\_\_a\_\_a\_" (replace underscores with any characters to reach exactly 12). Verify the total length and the 1-based indices before outputting.

\medskip
\promptheading{Word Counting \& Positioning:}\\
1. The checker splits text by spaces to count words. A comma or period attached to a word (e.g., "word,") counts as part of that word.\\
2. Punctuation attached to required words causes failures. If the 4th word must be "appealing", do not write "appealing,". The 4th space-separated token must be exactly "appealing".\\
3. If a position constraint seems to break natural grammar, prioritize the exact constraint. For example, if the 4th word must be "appealing", write: "The new design appealing is..." Do not force incorrect words into the required slots.\\
4. Mentally substitute required words into their exact positions first, then fill the remaining slots with placeholder words to meet the exact count. Example for 15 words (4th='for', 8th='sports', 11th='boxing'): "One two three for five six seven sports nine ten boxing twelve thirteen fourteen fifteen." Adjust the placeholders to form a sentence, but never alter the required words or their positions. Verify the final space-separated token indices before finishing.

\medskip
\promptheading{Format:}\\
1. Output strictly the requested text.\\
2. Do not include any preamble, conversational filler, labels, explanations, or quotation marks unless they are explicitly requested as part of the text.\\
3. Begin your response immediately with the first word of the requested text and end immediately after the final character.
\end{promptbox}

\begin{promptbox}{GEPA: 5 words, test 68.3\% (the unchanged seed)}
\small\ttfamily\raggedright\sloppy
You are a helpful assistant.
\end{promptbox}

\begin{promptbox}{OPRO: 20 words, test 71.5\%}
\small\ttfamily\raggedright\sloppy
Output only the exact text that meets the user's constraints perfectly. Do not add any extra words, introductions, or explanations.
\end{promptbox}

\begin{promptbox}{MIPROv2: 68 words, test 71.5\%}
\small\ttfamily\raggedright\sloppy
Each request asks for a piece of text (passage, paragraph, sentence or words) under exact structural constraints: word counts, sentence counts, required last/first sentences, specific words at specific positions, required or forbidden words. A program checks the constraint exactly; the reply scores 1 only if every stated condition holds, else 0. Replies must contain ONLY the requested text: any preamble or commentary becomes part of what is checked.
\end{promptbox}

\begin{promptbox}{GrIPS: 10 words, test 68.3\%}
\small\ttfamily\raggedright\sloppy
You are a helpful assistant. You are a supportive aid.
\end{promptbox}

\begin{promptbox}{aPSF: 117 words, test 71.5\%}
\small\ttfamily\raggedright\sloppy
Interpret the request as a strict formal puzzle with zero tolerance for deviations. Your sole job is to output only the exact text that satisfies every structural constraint perfectly, treating word counts, sentence counts, positional requirements, and term inclusions as immutable rules.\\
Count words and sentences carefully using standard definitions, treating punctuation normally. Verify start/end phrasing and required positional terms before finalizing. Validate every constraint condition.\\
Provide only the requested text with no preamble, explanation, or commentary. Formatting marks like Markdown are forbidden unless explicitly demanded by the prompt.\\
Honor absolute limits on word counts, sentence counts, opening and closing sentences, and inclusion or exclusion of specific words. If any single constraint is broken, the evaluation fails.
\end{promptbox}


\clearpage
\subsection{StackEval}

\begin{promptbox}{\method: 162 words, test 78.3\%}
\small\ttfamily\raggedright\sloppy
You are an automated task-solving assistant. Your output will be scored by a program that checks for 1 to 20 strict constraints related to formatting, length, wording, structure, required sections, and content.

\medskip
To maximize your score, follow these exact steps:

\medskip
1. \promptlabel{Analyze Constraints}: Scan the user request for a list of constraints. Treat every formatting and length requirement literally (e.g., exact starting words, max word count, specific keys in a JSON object, Markdown formatting).\\
2. \promptlabel{Plan Content}: Derive the core answer by directly addressing the prompt's topic, ensuring the content is relevant and complete without adding unnecessary filler.\\
3. \promptlabel{Execute Formatting}: Construct your response to satisfy all structural constraints simultaneously. Do not add conversational filler, introductory text, or labels like "answer:" unless explicitly requested.\\
4. \promptlabel{Validate}: Before finalizing, re-read the requested constraints and verify your output matches them exactly.

\medskip
\promptheading{\promptlabel{Format Execution Rules}:}\\
- If a JSON output is required, output only valid, parseable JSON. Do not include Markdown code blocks (e.g., no
\end{promptbox}

\begin{promptbox}{GEPA: 5 words, test 78.0\% (the unchanged seed)}
\small\ttfamily\raggedright\sloppy
You are a helpful assistant.
\end{promptbox}

\begin{promptbox}{OPRO: 40 words, test 77.5\%}
\small\ttfamily\raggedright\sloppy
You must follow all constraints in the prompt exactly. Pay close attention to every rule regarding format, length, wording, structure, required sections, and content. Output only the exact requested material. Do not include any introductions, conclusions, explanations, or filler text.
\end{promptbox}

\clearpage
\begin{promptbox}{MIPROv2: 227 words, test 74.1\%}
\small\ttfamily\raggedright\sloppy
You are a set completion model that predicts missing items from a constrained universe of alphanumeric IDs. The universe consists of 22 items across 6 categories (C, F, L, R, S, X), each with up to 4 numeric variants (e.g., C1, C2, C3, C4, F1, F2, ..., X4). Note that C2 and C3 are consistently absent and should never appear in your output.

\medskip
Given a request containing a set of observed items (sorted alphabetically then numerically, ranging from 1 to 20 items), your task is to predict which additional items from the universe should co-occur with the given set. The co-occurrence patterns are context-dependent, meaning the distributional characteristics governing which items belong together may shift across different batches or segments of data.

\medskip
Key considerations:\\
1. Only output items from the defined 22-item universe (excluding C2 and C3).\\
2. Items should be sorted alphabetically by category letter, then numerically within each category.\\
3. The output set size (including the input items) should be between 1 and 20 items total.\\
4. Learn from the observed items which distributional segment you are in, and predict the missing items that most likely co-occur.\\
5. If no additional items are predicted, return an empty set.

\medskip
Format your reply in the `[[ \#\# reply \#\# ]]` field as a comma-separated list of items, then conclude with the `[[ \#\# completed \#\# ]]` marker.
\end{promptbox}

\begin{promptbox}{GrIPS: 14 words, test 77.3\%}
\small\ttfamily\raggedright\sloppy
Serve as a supportive and useful guide. Act as a helpful and reliable resource.
\end{promptbox}

\begin{promptbox}{aPSF: 136 words, test 74.9\%}
\small\ttfamily\raggedright\sloppy
Your primary objective is to analyze the user's input and fulfill their underlying intent. Carefully determine the core subject matter and the exact action required before generating any text.\\
First, isolate the core subject and required action from the user's input. Next, mentally outline the necessary steps and gather relevant facts. Finally, verify that all compiled information is accurate and strictly aligned with the established goal before generating your response.\\
Structure your final response using clear markdown formatting, including appropriate headings and bullet points where applicable. Keep the language concise and ensure the total output remains under 200 words.\\
Strictly adhere to the specific list of provided constraints, as an automated program will evaluate your response for exact compliance. Failing to meet any of these formatting, length, or content rules will directly lower your evaluation score.
\end{promptbox}

\clearpage
\section{Prompts Written by the Swapped Optimizer}
\label{app:optswap_prompts}

Table~\ref{tab:optswap} reports what happens when GLM-5-FP8 is replaced by Qwen-3.5-27B as the optimizer.  The prompts below are what the swapped optimizer wrote for \method{} on the primary subject at seed 0, budget 250, and can be read against the GLM-5-FP8 versions earlier in this appendix.

\begin{promptbox}{HotpotQA, optimizer Qwen-3.5-27B (249 words, test 69.8\%)}
\small\ttfamily\raggedright\sloppy
You are a strict text-extraction engine. Your sole goal is to output the exact minimal text span that answers the question, maximizing token overlap with a gold standard. Every extra character, including newlines, prefixes, or explanations, incurs a penalty.

\medskip
\promptheading{STRATEGY:}\\
1. Identify the specific entity or fact requested.\\
2. Scan all paragraphs to locate the sentence containing the answer; ignore distractors.\\
3. Isolate the minimal contiguous substring that fully answers the question.\\
4. If the answer is a date, name, or number, extract ONLY those characters.\\
5. DO NOT infer, complete partial sentences, or include surrounding punctuation unless it is part of the specific answer entity (e.g., keep "1955" not "1955.").

\medskip
\promptheading{FORMAT:}\\
- Output the raw answer string ONLY.\\
- ZERO introductory text (e.g., "The answer is", "Based on text").\\
- ZERO concluding text, explanations, or citations.\\
- ZERO labels like "Answer:".\\
- ZERO Markdown formatting (no bold, no quotes, no code blocks).\\
- ZERO extra newlines or whitespace.\\
- The response must be the answer span and nothing else.

\medskip
\promptheading{CRITICAL RULES FOR HIGH SCORES:}\\
- If the answer is "15 December", output exactly "15 December". Never output "15 December\textbackslash{}n\textbackslash{}nAnswer: 15 December".\\
- If the answer is "Sri Lanka national cricket team", output exactly that. Never wrap in HTML or quotes.\\
- If the answer is "No", output exactly "No". Never add "Answer: No" or context about championships.\\
- Do not repeat the answer. Do not add periods if the source span didn't require them for the answer entity.
\end{promptbox}

\clearpage
\begin{promptbox}{IFBench, optimizer Qwen-3.5-27B (186 words, test 65.0\%)}
\small\ttfamily\raggedright\sloppy
You are an assistant that solves tasks while strictly adhering to every output constraint. Before generating your final response, perform this internal checklist:

\medskip
1. \promptlabel{Analyze Constraints}: Identify all explicit constraints in the user prompt (e.g., exact word counts, forbidden words, required formatting like `\promptlabel{**highlighted**}` or code blocks, case requirements like ALL CAPS, sentence counts, or specific repetition rules).\\
2. \promptlabel{Derive Content}: Solve the core problem (math, logic, translation) accurately based on the input facts.\\
3. \promptlabel{Format Enforcement}: Construct the final output to match the constraints *exactly*.\\
   - If "All Caps" is required, the *entire* response (including any intro/outro) must be uppercase.\\
   - If specific formatting (like highlighting sections) is required, apply it precisely.\\
   - If forbidden words are listed, ensure they do not appear anywhere.\\
   - If word counts or sentence structures are specified, count and adjust strictly.\\
4. \promptlabel{Final Verification}: Review the generated text one last time to ensure no constraint was missed or partially met.

\medskip
Output ONLY the final response that satisfies all constraints. Do not include explanations, reasoning steps, or meta-commentary in the final output unless explicitly requested as part of the constraints.
\end{promptbox}

\clearpage
\begin{promptbox}{StackEval, optimizer Qwen-3.5-27B (166 words, test 78.4\%)}
\small\ttfamily\raggedright\sloppy
You are a deterministic constraint-solver. Your sole objective is to maximize a programmatic score (0.0\promptdash{}1.0) by satisfying a hidden list of 1\promptdash{}20 output constraints. Conversational norms, helpfulness, and politeness are secondary; discard them if they conflict with any constraint.

\medskip
\promptheading{EXECUTE THIS PROTOCOL STRICTLY:}

\medskip
1. CONSTRAINT EXTRACTION \& VALIDATION\\
   - \promptlabel{Explicit Extraction}: Parse the prompt for exact quantifiers ("exactly N", "max N", "min N"), forbidden terms ("no X"), required formats (JSON, CSV, Markdown, plain text), and mandatory phrases.\\
   - \promptlabel{Implicit Deduction}: Infer strict requirements from context. If a structured format (e.g., JSON) is requested, syntax must be valid (balanced brackets, correct quoting). If a list size is implied by the data, match it exactly.\\
   - \promptlabel{Pre-Generation Simulation}: Before outputting, mentally run the checker against your planned response:\\
     * \promptlabel{Counts}: Verify word/character/sentence counts match the target exactly. Include spaces and punctuation in character counts. Do not round or approximate.\\
     * \promptlabel{Forbidden Tokens}: Ensure zero occurrences of forbidden elements (e.g., if "no markdown" is set, strip all `*`, `\#`,
\end{promptbox}

\clearpage
\begin{promptbox}{MBPP+, optimizer Qwen-3.5-27B (289 words, test 80.7\%)}
\small\ttfamily\raggedright\sloppy
You are a precision code generation engine for automated evaluation. Your sole objective is to output a self-contained Python code block that defines the exact function requested, matching the signature and logic required to pass both visible and hidden assertions.

\medskip
\promptheading{STRATEGY:}\\
1.  \promptlabel{Exact Signature Matching}: Extract the function name and parameter list strictly from the provided `assert` statements or explicit text.\\
    - If the request says `assert is\_samepatterns(["red"], ["a"])`, your definition MUST be `def is\_samepatterns(words, patterns):`.\\
    - Do NOT change parameter names (e.g., do not change `words` to `word\_list`), even if the variable names in the assert look like literals.\\
    - Do NOT add type hints or docstrings if they are not strictly required for logic, but ensure the signature matches exactly what the test harness expects.

\medskip
2.  \promptlabel{Logic Deduction via Assertion Analysis}:\\
    - Treat every provided `assert` as a ground-truth input-output pair.\\
    - Infer the algorithm by generalizing from these pairs. Look for:\\
        - Pattern matching (e.g., word-to-character mapping).\\
        - Edge cases (empty inputs, single elements, boundaries).\\
        - Return types (ensure the return value matches the `expected` value in the assert exactly, including type).\\
    - Prioritize correctness on hidden test cases by handling generic edge cases (e.g., returning `None` or `False` for invalid inputs if implied, or handling empty lists gracefully).

\medskip
3.  \promptlabel{Strict Self-Containment}:\\
    - The output must run in an isolated environment.\\
    - Import only standard library modules if absolutely necessary (e.g., `math`, `collections`). Do not import external packages.\\
    - Do not include any text, explanations, markdown outside the code block, or setup code (like `if \_\_name\_\_ == "\_\_main\_\_":`) that might interfere with the automated execution.

\medskip
\promptheading{FORMAT:}\\
1.  \promptlabel{Output Only Code}: Your entire response must be a single Python code block.\\
2.  \promptlabel{Structure}:\\
    - Start immediately with
\end{promptbox}


==> app_hotpot_feedback.tex <==
\section{HotpotQA Feedback Comparison}
\label{app:hotpot_feedback}

The paired failure-feedback experiment compares Full and the no-example arm on HotpotQA at seeds 0, 1 and 2.
Each arm and seed is run once, and all six outcomes are retained without score-based selection.

\paragraph{Matched protocol.}
Both arms use official HotpotQA answer-F1 normalization and its yes/no/noanswer mismatch rule, with prediction extraction from the last explicit answer label, or the last nonempty non-fence line when no label is present.
Simple wrapping markup is removed without consulting the gold answer.
The shared task description and user request explicitly allow yes/no answers.
A fixed 1\,200-row pool (pool seed 0, test-shuffle seed 999) provides the same 200 test questions for all six runs; run seeds vary the non-test split and search, with 150 training and 300 validation rows.
Dataset-native IDs verify split disjointness and common test content; the test questions match the seed-0 set used for the HotpotQA ablations in Table~\ref{tab:design}.

In Full, each of the first three failing slice rows shows the complete question, the first 240 characters of every context paragraph in input order, the extracted model answer, up to 800 trailing reply characters, and the row's F1.
Extracted answers exceeding 800 characters are shortened using their head and tail.
Gold answers and supporting-fact annotations are never shown to the optimizer.
The no-example arm differs only by omitting these examples from the same refinement template.
Both arms retain the primary subject, default optimizer and decoding settings, 16-row probe, adaptive fixed slice, two candidates per step, and greedy selection.
The optimization cap is 250 subject calls; actual use is 237--250 because only whole rounds are scheduled.
All six runs score all 200 test rows, and raw replies are retained for audit.

\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{7pt}
\caption{Per-seed HotpotQA results for the paired failure-example re-run (answer-F1 points, budget cap 250).  $\Delta$ is no examples minus the Full of this study, calculated before rounding.}
\label{tab:hotpot_feedback}
\begin{tabular}{l rrr}
\toprule
\rowcolor{headgray} \textbf{Seed} & \textbf{Full} & \textbf{No examples} & $\Delta$ \\
\midrule
0 & 81.27 & 81.61 & $+0.34$ \\
1 & 79.14 & 79.24 & $+0.10$ \\
2 & 80.51 & 82.25 & $+1.74$ \\
\midrule
\textbf{Mean} & \textbf{80.31} & \textbf{81.03} & \textbf{+0.73} \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Interpretation and aggregation.}
The no-example contrast is $+0.727$ points, positive in all three seeds (Table~\ref{tab:hotpot_feedback}); it does not establish a benefit from failure examples on HotpotQA.
The main HotpotQA experiment uses a local answer scorer and run-seed-dependent test pools, with 150-character request excerpts for failure feedback.
The paired feedback experiment instead uses official answer-F1, a common test set, explicit yes/no task wording, and the example representation above.
Its Full is therefore a study-specific reference: absolute HotpotQA scores should not be compared between this experiment and Table~\ref{tab:design}, and only the within-study contrast is meaningful.
This experiment is reported separately; its scores are not pooled with other protocols.


==> app_theory.tex <==
\section{Fixed-Pair Reliability and the Search Budget}
\label{app:theory}

This appendix gives a mechanism-level analysis of the evaluation design.  The statistical result concerns a fixed candidate pair on an independent sample, whereas the budget identity concerns Algorithm~\ref{alg:main}.  We keep these claims separate: combining a fixed-pair error bound with the call accounting does not establish a generalization guarantee for adaptively generated prompts.

\subsection{Comparison Model}
\label{app:theory_setup}

Fix an incumbent $p$, a candidate $c$, and a positive integer $s$ before observing the evaluation sample.  Let $(X_j,Y_j)_{j=1}^s$ be i.i.d. score pairs, where $X_j=f_{I_j}(c)$ and $Y_j=f_{I_j}(p)$ evaluate the two prompts on the same random row $I_j$.  Scores lie in $[0,1]$.  The probability law includes row sampling and, if the subject model is stochastic, its decoding randomness.  Within a row the two scores need not be independent; across rows the pairs are independent and identically distributed.  This is an idealized i.i.d. comparison, not an assumption that the implementation's probe-first, without-replacement slice has this law after calibration.

Write
\begin{align}
  Z_j &= X_j-Y_j, &
  \Delta &= \mathbb{E}[Z_j], \label{eq:theory_difference}\\
  \widehat\Delta_s &= \frac{1}{s}\sum_{j=1}^s Z_j, &
  v &= \mathrm{Var}(Z_j). \label{eq:theory_variance}
\end{align}
Here $\Delta$ is the difference of population mean scores under this evaluation law, not an observed slice or test-set difference.  With $\sigma_c^2=\mathrm{Var}(X_j)$, $\sigma_p^2=\mathrm{Var}(Y_j)$ and $\gamma_{cp}=\mathrm{Cov}(X_j,Y_j)$, expansion of the variance gives
\begin{equation}
  v=\sigma_c^2+\sigma_p^2-2\gamma_{cp},\qquad
  \mathrm{Var}(\widehat\Delta_s)=\frac{v}{s}.
  \label{eq:theory_pairing}
\end{equation}
If both marginal variances are positive, $\gamma_{cp}=\rho_{cp}\sigma_c\sigma_p$, where $\rho_{cp}$ is the same-row Pearson correlation.  The covariance form also covers zero marginal variance, for which that correlation is undefined.  Independent evaluation samples with the same marginals have $\gamma_{cp}=0$.  Thus pairing lowers the variance when $\gamma_{cp}>0$, leaves it unchanged when $\gamma_{cp}=0$, and can increase it when $\gamma_{cp}<0$.

This comparison holds the number of observations per prompt fixed.  It does not assume shared decoding randomness or assert that score covariance is positive for every prompt pair.  The Spearman correlation in Appendix~\ref{app:gengap} measures a different relationship, between search fitness and held-out performance across prompts, and is not an estimate of $\rho_{cp}$.

\subsection{The Comparison Bound}

\begin{proposition}[Fixed-pair comparison]
\label{prop:paired_error}
If $\Delta=\mathbb{E}[\widehat\Delta_s]>0$ and scores lie in $[0,1]$, the better candidate is rejected with probability
\begin{equation}
  \Pr(\widehat\Delta_s\leq0)
  \leq \exp\!\left(-\frac{s\Delta^2}{2v+\frac43\Delta}\right).
  \label{eq:misrank}
\end{equation}
\end{proposition}

This is a Bernstein bound~\citep{maurer2009empirical}: it ties pairing to decision reliability, and inverting it prices precision in refinement steps, since $T(s)$ is non-increasing (Corollary~\ref{cor:budget_precision}).

\paragraph{Proof of Proposition~\ref{prop:paired_error}.}
Suppose $\Delta>0$ and let $W_j=\Delta-Z_j$.  Then $\mathbb{E}[W_j]=0$, $\mathrm{Var}(W_j)=v$, and $|W_j|\leq2$ because $Z_j\in[-1,1]$.  Bernstein's exponential-moment bound for bounded, centered variables yields, for $0<\lambda<3/2$,
\begin{equation}
  \log\mathbb{E}\exp(\lambda W_j)
  \leq \frac{\lambda^2v}{2(1-2\lambda/3)}.
  \label{eq:theory_mgf}
\end{equation}
For completeness, expand the exponential and use $\mathbb{E}|W_j|^m\leq2^{m-2}v$ and $m!\geq2\cdot3^{m-2}$ for $m\geq2$; summing the resulting geometric series and applying $\log(1+x)\leq x$ gives Equation~\ref{eq:theory_mgf}.  This is the standard variance-sensitive concentration argument underlying Bernstein-type bounds~\citep{maurer2009empirical}.

Independence across rows and the exponential Markov inequality now give
\begin{align}
  \Pr(\widehat\Delta_s\leq0)
  &=\Pr\!\left(\sum_{j=1}^s W_j\geq s\Delta\right) \notag\\
  &\leq\exp\!\left[-\lambda s\Delta
       +\frac{s\lambda^2v}{2(1-2\lambda/3)}\right].
  \label{eq:theory_chernoff}
\end{align}
For $v>0$, substitute $\lambda=\Delta/(v+2\Delta/3)$ to obtain Equation~\ref{eq:misrank}.  If $v=0$, each $Z_j=\Delta>0$ almost surely, so the rejection probability is zero and the bound still holds.\hfill$\square$

The same argument applied to $-Z_j$ bounds erroneous acceptance when $\Delta<0$: $\Pr(\widehat\Delta_s>0)$ is at most the right-hand side of Equation~\ref{eq:misrank} with $\Delta$ replaced by $|\Delta|$.  There is no positive-margin guarantee at $\Delta=0$.  For fixed $\Delta>0$ and $s$, positive same-row covariance decreases the upper bound through $v$; a tighter bound alone does not establish a universal ordering of the actual error probabilities.

\subsection{A Sufficient Precision Target and Its Budget Cost}

\begin{corollary}[Budget cost]
\label{cor:budget_precision}
Under Proposition~\ref{prop:paired_error}, fix $\delta\in(0,1)$, $\Delta>0$, and $v$.  For integer slice limits define
\begin{equation}
  s_{\mathrm{cert}}=
  \max\!\left\{s_{\min},
  \left\lceil\frac{2v+\frac43\Delta}{\Delta^2}
  \log\frac{1}{\delta}\right\rceil\right\}.
  \label{eq:slice_certificate}
\end{equation}
If $s_{\mathrm{cert}}\leq s_{\max}$, evaluating the fixed pair on $s_{\mathrm{cert}}$ i.i.d. rows makes its rejection-error bound at most $\delta$.  Under the call accounting of Equation~\ref{eq:steps}, this size also permits at least one complete refinement step if
\begin{equation}
  n_\text{probe}+(\ncand+1)s_{\mathrm{cert}}\leq B.
  \label{eq:certificate_feasibility}
\end{equation}
When both conditions hold, $s_{\mathrm{cert}}$ maximizes the number of affordable complete steps among permitted integer slice sizes satisfying this sufficient certificate.
\end{corollary}

\paragraph{Proof of Corollary~\ref{cor:budget_precision}.}
Requiring the right-hand side of Equation~\ref{eq:misrank} to be at most $\delta$ gives
\begin{equation}
  s\geq\frac{2v+\frac43\Delta}{\Delta^2}\log\frac{1}{\delta}.
  \label{eq:certificate_requirement}
\end{equation}
Equation~\ref{eq:slice_certificate} is the smallest permitted integer satisfying this sufficient inequality.  After the probe and seed scoring, one complete step costs $\ncand s$ calls, giving Equation~\ref{eq:certificate_feasibility}.  Finally,
\begin{equation}
  T(s)=\left\lfloor
      \frac{B-n_\text{probe}}{\ncand s}-\frac{1}{\ncand}
      \right\rfloor
  \label{eq:theory_steps}
\end{equation}
is non-increasing in $s$ on the feasible domain.  The smallest certified size therefore attains the largest $T(s)$ within that domain, possibly tied with larger sizes.\hfill$\square$

This is an oracle comparison: $v$ and $\Delta$ are population quantities, not inputs known to \method.  The certificate is sufficient rather than necessary, and can be conservative; when $v=0$, for example, the comparison has zero error even without this certificate.  If $s_{\mathrm{cert}}>s_{\max}$ or Equation~\ref{eq:certificate_feasibility} fails, no permitted size both satisfies this particular certificate and funds a complete step.  That does not prove that reliable comparison or useful optimization is impossible.  Nor does maximizing affordable steps imply maximizing final performance: the quality of future proposals is not modeled here.

\subsection{Relation to the Implemented Rule}

Equation~\ref{eq:se} motivates $s\approx\sigma^2/\tse^2$ for estimating one fixed prompt's mean.  Equation~\ref{eq:slice_certificate} instead concerns a particular comparison and depends on its gap and difference variance.  The seed-probe estimate $\hat\sigma^2$ is neither $v$ nor a confidence upper bound on future candidates' variances.  Consequently, substituting $\hat\sigma$ into Equation~\ref{eq:slice} does not inherit Corollary~\ref{cor:budget_precision}'s error target.  Small probes, changing candidate variances, integer rounding, and the slice limits all affect this proxy.

There is a second distinction: Algorithm~\ref{alg:main} chooses $s$ from the probe and includes probe rows in $S$; subsequent candidates depend on scores and failing examples from $S$.  Conditioning on those choices does not restore the fixed-pair i.i.d. setup.  A guarantee uniform over the whole adaptive search would require additional control, for example a uniform bound over a prespecified prompt class or an adaptive-data-analysis argument~\citep{dwork2015holdout}.  Simply applying the fixed-pair bound to the realized candidate count and taking a union bound is not justified.

\paragraph{Algorithmic invariants.}
Under the row-call accounting of Algorithm~\ref{alg:main}, assuming $B\geq n_\text{probe}+s$ and complete evaluation of all $\ncand$ proposals in every executed step, $t$ steps cost
\begin{equation}
  B_{\mathrm{used}}=n_\text{probe}+s+t\ncand s\leq B.
  \label{eq:theory_accounting}
\end{equation}
The loop guard establishes the inequality by induction; if termination is solely due to the guard, fewer than $\ncand s$ calls remain.  Strict acceptance also makes the incumbent's \emph{recorded slice score} non-decreasing, since a candidate replaces it only when that score increases.  Neither invariant guarantees an increase in the population or held-out score, and the accounting statement does not verify any baseline's implementation.

The analysis therefore supports a design principle, not an optimality claim: pairing can reduce comparison variance, while finer evaluation reduces search capacity.  Whether the seed-based proxy chooses a useful balance in an adaptive run is addressed by the measured ablations and budget sweeps, with held-out diagnostics in Appendix~\ref{app:gengap}.


==> gengap_summary.tex <==
% Generated by build_fig_gengap.py from plotted test-half-B scores.
\newcommand{\gengapCells}{35}
\newcommand{\gengapDefined}{34}
\newcommand{\gengapMean}{+0.14}
\newcommand{\gengapMedian}{+0.20}
\newcommand{\gengapPositive}{21}
\newcommand{\gengapStrongPositive}{13}
\newcommand{\gengapStrongNegative}{4}
\newcommand{\gengapMinCandidates}{9}
\newcommand{\gengapMaxCandidates}{13}


==> prompt_style.tex <==
% Prompt exhibits. The unmodified framed.sty is vendored from CTAN:
% https://ctan.org/pkg/framed (v0.96; license notice retained in that file).
\usepackage{framed}
\definecolor{PromptFrame}{RGB}{210,227,232}
\definecolor{PromptAccent}{RGB}{33,88,102}
\colorlet{TFFrameColor}{PromptFrame}
\colorlet{TFTitleColor}{PromptAccent}
\newlength{\PromptTitleWidth}

\newcommand{\PromptFrameBlock}[2]{%
  \begingroup
  \fboxsep=12pt\fboxrule=0.8pt
  \TitleBarFrame{%
    \parbox{\PromptTitleWidth}{%
      \normalfont\rmfamily\fontsize{11}{14}\selectfont\bfseries
      \strut #1\strut}}{#2}%
  \endgroup
}

\newenvironment{promptbox}[1]{%
  \par\begingroup
  % Disable lineno's forced interline breaks inside the split exhibit box.
  \nolinenumbers
  \color{black}%
  \setlength{\PromptTitleWidth}{\dimexpr\linewidth-25.6pt\relax}%
  \setlength{\OuterFrameSep}{12pt}%
  \def\FrameCommand##1{\PromptFrameBlock{#1}{##1}}%
  \def\FirstFrameCommand##1{\PromptFrameBlock{#1}{##1}}%
  \def\MidFrameCommand##1{\PromptFrameBlock{#1\quad\normalfont\itshape(continued)}{##1}}%
  \let\LastFrameCommand\MidFrameCommand
  \MakeFramed{\advance\hsize-25.6pt\FrameRestore}%
  \def\small{\fontsize{10}{13}\selectfont}%
  \small\ttfamily\raggedright
  \setlength{\parindent}{0pt}%
  \setlength{\parskip}{5pt}%
  \hyphenpenalty=10000\exhyphenpenalty=10000
  \emergencystretch=2em
}{%
  \par\endMakeFramed\endgroup\color{black}%
}

\newcommand{\promptheading}[1]{{\color{PromptAccent}\bfseries #1}}
\newcommand{\promptlabel}[1]{{\bfseries #1}}
\newcommand{\promptdash}{{\normalfont\textendash}}


==> tab_bench.tex <==
\footnotesize
\setlength{\tabcolsep}{4.6pt}
\renewcommand{\arraystretch}{1.35}
\begin{tabular}{lccccccc|c}
\toprule
\rowcolor{headgray} \textbf{Method} & \textbf{Hotpot} & \textbf{CollIE} & \textbf{IFBench} & \textbf{SuperGPQA} & \textbf{Stack} & \textbf{MBPP+} & \textbf{LB-IF} & \textbf{Mean} \\
\midrule
\emph{No opt.} & 61.50 & 52.80 & 44.80 & 42.60 & 71.37 & 76.53 & 63.26 & 58.98 \\
\rowcolor{bandblue!8} \multicolumn{9}{l}{\textcolor{bandblue}{\textit{Published baselines}}} \\
GEPA & 64.60{\scriptsize$\pm$12.91} & 54.02{\scriptsize$\pm$14.15} & 46.12{\scriptsize$\pm$9.05} & 42.37{\scriptsize$\pm$12.79} & 71.29{\scriptsize$\pm$6.65} & \bfirst{77.41}{\scriptsize$\pm$4.47} & 63.72{\scriptsize$\pm$6.22} & 59.93 \\
OPRO & 67.55{\scriptsize$\pm$11.29} & 57.30{\scriptsize$\pm$15.61} & 50.58{\scriptsize$\pm$11.16} & 44.13{\scriptsize$\pm$10.38} & \usecond{71.85}{\scriptsize$\pm$6.11} & 75.42{\scriptsize$\pm$4.16} & \usecond{63.97}{\scriptsize$\pm$5.46} & \usecond{61.54} \\
MIPROv2 & \usecond{69.79}{\scriptsize$\pm$12.83} & 57.60{\scriptsize$\pm$15.27} & 50.75{\scriptsize$\pm$12.05} & 42.43{\scriptsize$\pm$12.75} & 69.17{\scriptsize$\pm$7.36} & 74.47{\scriptsize$\pm$4.02} & 63.00{\scriptsize$\pm$7.66} & 61.03 \\
GrIPS & 66.15{\scriptsize$\pm$11.52} & 52.92{\scriptsize$\pm$13.63} & 47.15{\scriptsize$\pm$9.34} & 42.07{\scriptsize$\pm$12.63} & 70.92{\scriptsize$\pm$6.69} & 76.10{\scriptsize$\pm$4.86} & 63.13{\scriptsize$\pm$6.23} & 59.78 \\
aPSF & 69.25{\scriptsize$\pm$8.54} & \usecond{58.10}{\scriptsize$\pm$15.85} & \bfirst{52.85}{\scriptsize$\pm$11.04} & \usecond{44.18}{\scriptsize$\pm$10.73} & 69.55{\scriptsize$\pm$6.62} & 70.64{\scriptsize$\pm$7.76} & 63.49{\scriptsize$\pm$5.97} & 61.15 \\
\cdashline{1-9}
\rowcolor{oursrow} \method & \bfirst{73.29}{\scriptsize$\pm$8.85} & \bfirst{59.50}{\scriptsize$\pm$17.40} & \usecond{52.00}{\scriptsize$\pm$11.01} & \bfirst{45.33}{\scriptsize$\pm$11.54} & \bfirst{73.00}{\scriptsize$\pm$5.02} & \usecond{77.30}{\scriptsize$\pm$4.14} & \bfirst{64.23}{\scriptsize$\pm$6.11} & \bfirst{63.52} \\
\midrule
\emph{Baseline spread} & 5.19 & 5.18 & 6.73 & 2.11 & 2.68 & 6.77 & 0.97 & 1.76 \\
\bottomrule
\end{tabular}


==> tab_budget.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.25}
\caption{\textbf{Budget curve, full range.}  Mean test score (\%) over the seven benchmarks and three seeds, GPT-OSS-20B.  Figure~\ref{fig:teaser}(a) draws 100--400; 450 and 500 are here.  \method and GEPA converge past 400.}
\label{tab:app_budget}
\begin{tabular}{lccccccccc}
\toprule
\rowcolor{headgray} \textbf{Method} & 100 & 150 & 200 & 250 & 300 & 350 & 400 & 450 & 500 \\
\midrule
\method & 64.9 & 67.0 & 65.7 & 65.2 & 66.2 & 66.4 & 65.6 & 64.4 & 65.1 \\
GEPA & 59.2 & 59.3 & 59.9 & 60.1 & 60.0 & 64.3 & 64.3 & 65.0 & 65.2 \\
OPRO & 61.2 & 61.9 & 62.7 & 63.2 & 63.0 & 62.6 & 63.0 & 64.3 & 63.3 \\
MIPROv2 & 62.9 & 62.9 & 61.9 & 63.8 & 64.4 & 63.8 & 63.8 & 62.6 & 64.9 \\
GrIPS & 58.5 & 58.7 & 59.4 & 59.4 & 59.5 & 59.6 & 59.0 & 58.9 & 59.3 \\
aPSF & 65.0 & 63.5 & 65.2 & 62.4 & 65.4 & 65.0 & 63.7 & 64.1 & 65.0 \\
\bottomrule
\end{tabular}
\end{table}


==> tab_design.tex <==
\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{6.2pt}
\caption{Ablations and hyper-parameter sweeps, primary subject (\%, budget 250); each column changes one thing, read against the shaded \textbf{Full} entry.  $-$Adapt.: fixed $s{=}20$, probe still spent.  $-$Fixed: slice redrawn every step, incumbent re-scored on it.  $-$Strat.: plain ``raise the score'' request, no failing rows.  $-$Fail.: strategy and format kept, no failing rows.  Otherwise $\tse{=}0.10$, $\ncand{=}2$.}
\label{tab:design}
\begin{tabular}{l|>{\columncolor{ourstint}}c|cccc|ccc|cc}
\toprule
\rowcolor{headgray} & \textbf{Full} & \multicolumn{4}{c|}{\textbf{Ablation (remove one)}} & \multicolumn{3}{c|}{\textbf{Target SE}} & \multicolumn{2}{c}{\textbf{Cand./step}} \\
\rowcolor{headgray} \textbf{Benchmark} & \method & $-$Adapt. & $-$Fixed & $-$Strat. & $-$Fail. & $\tse{=}.05$ & $\tse{=}.15$ & $\tse{=}.20$ & $\ncand{=}1$ & $\ncand{=}3$ \\
\midrule
HotpotQA & 74.3 & 66.1 & 65.9 & 68.8 & 73.2 & 65.0 & 61.5 & 60.9 & 74.9 & 68.9 \\
CollIE & 74.2 & 70.8 & 72.7 & 69.8 & 70.0 & 72.8 & 70.2 & 71.2 & 71.8 & 73.0 \\
IFBench & 62.7 & 62.7 & 65.2 & 61.2 & 63.6 & 62.8 & 63.1 & 61.8 & 63.9 & 62.7 \\
SuperGPQA & 60.5 & 61.2 & 61.5 & 62.5 & 62.5 & 63.0 & 62.3 & 62.0 & 60.0 & 61.0 \\
StackEval & 78.7 & 78.7 & 78.6 & 77.7 & 77.5 & 78.1 & 78.3 & 78.5 & 77.8 & 77.7 \\
MBPP+ & 81.3 & 81.1 & 79.3 & 81.1 & 80.2 & 81.8 & 80.4 & 81.6 & 80.2 & 80.9 \\
LiveBenchIF & 69.2 & 68.3 & 68.5 & 68.7 & 67.6 & 68.4 & 68.7 & 68.8 & 68.9 & 68.1 \\
\midrule
\textbf{Mean} & \textbf{71.6} & 69.8 & 70.2 & 70.0 & 70.7 & 70.3 & 69.2 & 69.2 & 71.1 & 70.3 \\
\bottomrule
\end{tabular}
\end{table*}


==> tab_escape.tex <==
\begin{table}[t]
\centering
\scriptsize
\renewcommand{\arraystretch}{1.62}
\setlength{\tabcolsep}{4.4pt}
\caption{\textbf{Seed return} (\%) by subject under a 250-call cap; 21 runs per cell, 105 per method.  Returned prompts are compared with the seed after trimming leading and trailing whitespace.  MIPROv2 and aPSF always rewrite.}
\label{tab:escape}
\begin{tabular}{lcccccc}
\toprule
\rowcolor{headgray} \textbf{Method} & \textbf{Gemma} & \textbf{GPT-OSS} & \textbf{Qwen} & \textbf{Nemo.} & \textbf{Minis.} & \textbf{All} \\
\midrule
\rowcolor{ourstint} \method & 5 & 10 & 24 & 14 & 14 & 13 \\
GEPA & 71 & 81 & 90 & 90 & 95 & 86 \\
OPRO & 33 & 5 & 43 & 19 & 19 & 24 \\
GrIPS & 14 & 10 & 19 & 19 & 19 & 16 \\
MIPROv2 & 0 & 0 & 0 & 0 & 0 & 0 \\
aPSF & 0 & 0 & 0 & 0 & 0 & 0 \\
\bottomrule
\end{tabular}
\end{table}


==> tab_main_big.tex <==
\begin{table*}[!t]
\centering
\scriptsize
\setlength{\tabcolsep}{2.6pt}
\caption{\textbf{Main result per cell.}  Test score (\%) at a 250-call cap, mean$_{\pm\text{std}}$ over seeds 0/1/2, with sample standard deviations.  Within each subject, all methods share the optimizer (GLM-5-FP8), budget, decoding and seed prompt.  \emph{No optimization}: archived seed-0 reference evaluations.  \textbf{Bold}: the column's best in the block and every entry within one standard error of that best entry; this is a display rule, with significance tested separately in Table~\ref{tab:sig}.  Shaded: \method, its margin over the block's best baseline in \textcolor{gaingreen}{green}.}
\label{tab:main_big}
\begin{tabular}{llccccccc|c}
\toprule
\textbf{Subject} & \textbf{Method} & \textbf{Hotpot} & \textbf{CollIE} & \textbf{IFBench} & \textbf{SuperGPQA} & \textbf{Stack} & \textbf{MBPP+} & \textbf{LB-IF} & \textbf{Avg} \\
\midrule
\midrule
\multicolumn{9}{l}{\textit{Subject = Gemma-4-31B}} \\
\addlinespace[1pt]
 & \emph{No optimization} & 50.56 & 67.50 & 57.75 & 61.00 & 77.41 & 77.33 & 67.37 & 65.56 \\
\addlinespace[1pt]
 & GEPA & 54.31{\tiny$\pm$3.91} & 69.45{\tiny$\pm$1.78} & 57.83{\tiny$\pm$1.53} & \bfirst{61.83}{\tiny$\pm$0.58} & 77.79{\tiny$\pm$0.32} & \bfirst{80.44}{\tiny$\pm$1.39} & 68.10{\tiny$\pm$1.42} & 67.11 \\
 & OPRO & 52.00{\tiny$\pm$3.00} & 71.67{\tiny$\pm$1.26} & 63.92{\tiny$\pm$1.13} & 60.50{\tiny$\pm$1.73} & 77.96{\tiny$\pm$1.02} & 79.33{\tiny$\pm$2.00} & 67.64{\tiny$\pm$0.72} & 67.58 \\
 & MIPROv2 & 49.79{\tiny$\pm$4.45} & 70.67{\tiny$\pm$0.76} & 64.33{\tiny$\pm$1.88} & \bfirst{61.50}{\tiny$\pm$0.50} & 73.38{\tiny$\pm$4.66} & 79.33{\tiny$\pm$2.67} & 67.37{\tiny$\pm$0.05} & 66.62 \\
 & GrIPS & 57.12{\tiny$\pm$1.98} & 68.11{\tiny$\pm$0.20} & 56.92{\tiny$\pm$1.84} & 61.33{\tiny$\pm$1.26} & 77.46{\tiny$\pm$0.73} & \bfirst{80.89}{\tiny$\pm$1.02} & 66.92{\tiny$\pm$0.48} & 66.97 \\
 & aPSF & 62.71{\tiny$\pm$13.33} & 71.50{\tiny$\pm$1.00} & \bfirst{65.33}{\tiny$\pm$0.14} & \bfirst{62.33}{\tiny$\pm$1.53} & 75.58{\tiny$\pm$1.48} & 76.89{\tiny$\pm$2.34} & 67.60{\tiny$\pm$0.25} & 68.85 \\
\rowcolor{ourstint} & \method & \bfirst{74.34}{\tiny$\pm$6.03} & \bfirst{74.17}{\tiny$\pm$2.02} & 62.75{\tiny$\pm$3.70} & 60.50{\tiny$\pm$2.78} & \bfirst{78.67}{\tiny$\pm$0.31} & \bfirst{81.33}{\tiny$\pm$1.76} & \bfirst{69.24}{\tiny$\pm$1.37} & \bfirst{71.57}{\tiny\textcolor{gaingreen}{+2.72}} \\
\midrule
\multicolumn{9}{l}{\textit{Subject = GPT-OSS-20B}} \\
\addlinespace[1pt]
 & \emph{No optimization} & 68.13 & 66.00 & 42.75 & 36.00 & 65.13 & 72.00 & 61.62 & 58.80 \\
\addlinespace[1pt]
 & GEPA & 70.14{\tiny$\pm$2.72} & 68.67{\tiny$\pm$1.26} & 43.92{\tiny$\pm$0.63} & 35.00{\tiny$\pm$1.32} & 65.10{\tiny$\pm$0.91} & \bfirst{76.44}{\tiny$\pm$2.78} & 61.44{\tiny$\pm$0.96} & 60.10 \\
 & OPRO & \bfirst{73.87}{\tiny$\pm$2.90} & 78.00{\tiny$\pm$3.50} & 52.83{\tiny$\pm$7.04} & \bfirst{38.33}{\tiny$\pm$2.52} & 66.42{\tiny$\pm$1.63} & 70.89{\tiny$\pm$1.68} & \bfirst{62.19}{\tiny$\pm$0.24} & 63.22 \\
 & MIPROv2 & \bfirst{76.23}{\tiny$\pm$4.53} & 78.33{\tiny$\pm$5.06} & 53.17{\tiny$\pm$5.49} & 35.83{\tiny$\pm$2.08} & \bfirst{67.72}{\tiny$\pm$0.52} & 73.56{\tiny$\pm$2.78} & 61.77{\tiny$\pm$0.84} & 63.80 \\
 & GrIPS & 71.02{\tiny$\pm$3.22} & 67.17{\tiny$\pm$4.01} & 45.67{\tiny$\pm$1.01} & 34.83{\tiny$\pm$1.61} & 64.47{\tiny$\pm$1.34} & 71.33{\tiny$\pm$1.15} & 61.54{\tiny$\pm$0.52} & 59.43 \\
 & aPSF & 72.17{\tiny$\pm$5.65} & 80.00{\tiny$\pm$1.80} & \bfirst{58.17}{\tiny$\pm$3.02} & \bfirst{38.50}{\tiny$\pm$0.50} & 64.84{\tiny$\pm$1.83} & 61.11{\tiny$\pm$14.15} & \bfirst{62.05}{\tiny$\pm$0.59} & 62.41 \\
\rowcolor{ourstint} & \method & \bfirst{74.79}{\tiny$\pm$4.25} & \bfirst{83.67}{\tiny$\pm$1.44} & 54.42{\tiny$\pm$8.18} & 38.00{\tiny$\pm$1.50} & 66.97{\tiny$\pm$1.43} & \bfirst{76.22}{\tiny$\pm$3.79} & \bfirst{62.65}{\tiny$\pm$1.05} & \bfirst{65.24}{\tiny\textcolor{gaingreen}{+1.44}} \\
\midrule
\multicolumn{9}{l}{\textit{Subject = Qwen-3.5-27B}} \\
\addlinespace[1pt]
 & \emph{No optimization} & 69.62 & 50.00 & 51.50 & 52.00 & 78.93 & 80.67 & 67.24 & 64.28 \\
\addlinespace[1pt]
 & GEPA & 75.61{\tiny$\pm$4.46} & \bfirst{53.67}{\tiny$\pm$1.04} & 53.58{\tiny$\pm$0.95} & 51.67{\tiny$\pm$1.26} & \bfirst{79.14}{\tiny$\pm$0.47} & \bfirst{81.11}{\tiny$\pm$0.38} & 68.03{\tiny$\pm$0.77} & 66.11 \\
 & OPRO & 78.02{\tiny$\pm$2.52} & 51.83{\tiny$\pm$1.04} & 55.25{\tiny$\pm$2.88} & 50.00{\tiny$\pm$1.32} & 77.84{\tiny$\pm$1.65} & 79.11{\tiny$\pm$3.29} & 68.38{\tiny$\pm$0.18} & 65.78 \\
 & MIPROv2 & \bfirst{81.65}{\tiny$\pm$4.75} & \bfirst{53.00}{\tiny$\pm$3.28} & \bfirst{58.33}{\tiny$\pm$2.70} & 51.33{\tiny$\pm$1.26} & 77.47{\tiny$\pm$0.66} & 72.44{\tiny$\pm$1.54} & \bfirst{68.90}{\tiny$\pm$0.46} & 66.16 \\
 & GrIPS & 77.31{\tiny$\pm$5.34} & 50.33{\tiny$\pm$0.76} & 55.42{\tiny$\pm$1.81} & 50.83{\tiny$\pm$2.75} & 77.72{\tiny$\pm$0.60} & 79.11{\tiny$\pm$3.91} & 68.20{\tiny$\pm$0.35} & 65.56 \\
 & aPSF & 74.23{\tiny$\pm$4.55} & 52.33{\tiny$\pm$1.04} & \bfirst{57.92}{\tiny$\pm$0.76} & 48.67{\tiny$\pm$1.76} & 75.98{\tiny$\pm$0.86} & 72.00{\tiny$\pm$0.67} & 68.14{\tiny$\pm$0.98} & 64.18 \\
\rowcolor{ourstint} & \method & 77.25{\tiny$\pm$10.00} & \bfirst{54.17}{\tiny$\pm$2.57} & 56.75{\tiny$\pm$3.03} & \bfirst{56.33}{\tiny$\pm$1.04} & 78.54{\tiny$\pm$0.56} & 80.00{\tiny$\pm$0.67} & \bfirst{68.76}{\tiny$\pm$0.88} & \bfirst{67.40}{\tiny\textcolor{gaingreen}{+1.24}} \\
\midrule
\multicolumn{9}{l}{\textit{Subject = Nemotron-3-Super-120B}} \\
\addlinespace[1pt]
 & \emph{No optimization} & 72.63 & 43.00 & 40.25 & 29.00 & 72.46 & 81.33 & 68.09 & 58.11 \\
\addlinespace[1pt]
 & GEPA & \bfirst{76.54}{\tiny$\pm$3.48} & 43.17{\tiny$\pm$1.44} & 41.92{\tiny$\pm$0.72} & 29.50{\tiny$\pm$2.00} & 71.06{\tiny$\pm$1.03} & \bfirst{79.29}{\tiny$\pm$0.67} & \bfirst{68.07}{\tiny$\pm$0.48} & 58.51 \\
 & OPRO & 76.13{\tiny$\pm$4.33} & \bfirst{44.50}{\tiny$\pm$0.50} & 48.42{\tiny$\pm$1.61} & \bfirst{37.83}{\tiny$\pm$4.04} & \bfirst{72.68}{\tiny$\pm$1.98} & 76.22{\tiny$\pm$2.34} & 67.24{\tiny$\pm$0.18} & 60.43 \\
 & MIPROv2 & \bfirst{78.54}{\tiny$\pm$3.50} & \bfirst{44.50}{\tiny$\pm$2.50} & 46.08{\tiny$\pm$5.56} & 28.17{\tiny$\pm$4.04} & 70.15{\tiny$\pm$1.23} & 77.01{\tiny$\pm$3.63} & 67.14{\tiny$\pm$0.63} & 58.80 \\
 & GrIPS & 75.11{\tiny$\pm$2.90} & 43.33{\tiny$\pm$2.47} & 45.58{\tiny$\pm$2.74} & 30.00{\tiny$\pm$2.65} & \bfirst{72.58}{\tiny$\pm$0.43} & \bfirst{78.93}{\tiny$\pm$1.09} & 66.96{\tiny$\pm$0.45} & 58.93 \\
 & aPSF & 75.07{\tiny$\pm$4.49} & \bfirst{45.17}{\tiny$\pm$4.16} & 48.00{\tiny$\pm$2.17} & \bfirst{37.07}{\tiny$\pm$2.29} & 71.51{\tiny$\pm$0.72} & 73.66{\tiny$\pm$0.93} & 66.78{\tiny$\pm$0.74} & 59.61 \\
\rowcolor{ourstint} & \method & \bfirst{78.36}{\tiny$\pm$3.66} & \bfirst{45.17}{\tiny$\pm$2.47} & \bfirst{53.00}{\tiny$\pm$1.52} & \bfirst{38.67}{\tiny$\pm$5.01} & 70.45{\tiny$\pm$1.18} & 77.40{\tiny$\pm$3.70} & 66.94{\tiny$\pm$0.24} & \bfirst{61.43}{\tiny\textcolor{gaingreen}{+1.00}} \\
\midrule
\multicolumn{9}{l}{\textit{Subject = Ministral-8B}} \\
\addlinespace[1pt]
 & \emph{No optimization} & 46.56 & 37.50 & 31.75 & 35.00 & 62.94 & 71.33 & 51.96 & 48.15 \\
\addlinespace[1pt]
 & GEPA & 46.40{\tiny$\pm$3.81} & 35.17{\tiny$\pm$2.02} & 33.33{\tiny$\pm$0.63} & 33.83{\tiny$\pm$0.76} & 63.38{\tiny$\pm$0.32} & 69.78{\tiny$\pm$1.02} & 52.94{\tiny$\pm$0.61} & 47.83 \\
 & OPRO & 57.73{\tiny$\pm$2.66} & \bfirst{40.50}{\tiny$\pm$4.92} & 32.50{\tiny$\pm$2.25} & \bfirst{34.00}{\tiny$\pm$3.12} & 64.36{\tiny$\pm$3.42} & \bfirst{71.56}{\tiny$\pm$0.77} & \bfirst{54.39}{\tiny$\pm$0.40} & 50.72 \\
 & MIPROv2 & \bfirst{62.72}{\tiny$\pm$3.88} & \bfirst{41.50}{\tiny$\pm$3.28} & 31.83{\tiny$\pm$1.77} & \bfirst{35.33}{\tiny$\pm$2.31} & 57.13{\tiny$\pm$1.84} & 70.00{\tiny$\pm$0.00} & 49.83{\tiny$\pm$6.40} & 49.76 \\
 & GrIPS & 50.20{\tiny$\pm$5.56} & 35.67{\tiny$\pm$5.77} & 32.17{\tiny$\pm$2.40} & 33.33{\tiny$\pm$3.75} & 62.35{\tiny$\pm$0.43} & 70.22{\tiny$\pm$0.77} & 52.02{\tiny$\pm$0.32} & 47.99 \\
 & aPSF & \bfirst{62.05}{\tiny$\pm$4.17} & \bfirst{41.50}{\tiny$\pm$5.77} & \bfirst{34.83}{\tiny$\pm$1.46} & \bfirst{34.33}{\tiny$\pm$0.76} & 59.85{\tiny$\pm$1.92} & 69.56{\tiny$\pm$1.02} & 52.88{\tiny$\pm$1.16} & 50.72 \\
\rowcolor{ourstint} & \method & \bfirst{61.74}{\tiny$\pm$10.66} & \bfirst{40.33}{\tiny$\pm$1.04} & 33.08{\tiny$\pm$1.53} & 33.17{\tiny$\pm$0.29} & \bfirst{70.37}{\tiny$\pm$1.99} & \bfirst{71.56}{\tiny$\pm$1.39} & 53.59{\tiny$\pm$2.09} & \bfirst{51.98}{\tiny\textcolor{gaingreen}{+1.26}} \\
\bottomrule
\end{tabular}
\end{table*}


==> tab_xl.tex <==
\begin{table}[t]
\centering
\small
\caption{Enlarged test evaluations of the shipped prompts (primary subject, three seeds).  Scores combine original and additional rows without re-optimization.  Additional rows are shared across methods, with row-key exclusion as specified in the text.  $\Delta$: \method's margin over the strongest baseline.  The last three tasks retain their original evaluations.}
\label{tab:app_xl}
\setlength{\tabcolsep}{4.5pt}
\begin{tabular}{l rr rr}
\toprule
\textbf{Benchmark} & \textbf{Rows} & \textbf{Total} & $\Delta$ & $\Delta$ \textbf{enlarged} \\
\midrule
HotpotQA & 200 & 1000 & $+11.63$ & $+9.92$ \\
CollIE & 200 & 731 & $+2.50$ & $+1.46$ \\
SuperGPQA & 200 & 1000 & $-1.83$ & $-1.44$ \\
StackEval & 200 & 1000 & $+0.70$ & $+0.64$ \\
\midrule
\multicolumn{5}{l}{\emph{Original test evaluation only}} \\
IFBench & 200 & --- & $-2.58$ & --- \\
MBPP+ & 150 & --- & $+0.44$ & --- \\
LiveBenchIF & 150 & --- & $+1.13$ & --- \\
\bottomrule
\end{tabular}
\end{table}

